AgentNoiseBench: Benchmarking Robustness of Tool-Using LLM Agents Under Noisy Condition

Recent advances in large language models have enabled LLM-based agents to achieve strong performance on a variety of benchmarks. However, their performance in real-world deployments often that observed on benchmark settings, especially in complex and imperfect environments. This discrepancy largely arises because prevailing training and evaluation paradigms are typically built on idealized assumptions, overlooking the inherent stochasticity and noise present in real-world interactions. To bridge this gap, we introduce AgentNoiseBench, a framework for systematically evaluating the robustness of agentic models under noisy environments. We first conduct an in-depth analysis of biases and uncertainties in real-world scenarios and categorize environmental noise into two primary types: user-noise and tool-noise. Building on this analysis, we develop an automated pipeline that injects controllable noise into existing agent-centric benchmarks while preserving task solvability. Leveraging this pipeline, we perform extensive evaluations across a wide range of models with diverse architectures and parameter scales. Our results reveal consistent performance variations under different noise conditions, highlighting the sensitivity of current agentic models to realistic environmental perturbations.

==> exp/exp1_version2.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}

\textbf{Model Zoo.} 
We evaluate a curated set of 21 state-of-the-art large language models with more than 32B parameters, selected to cover diverse model architectures and training paradigms. 
To examine the effect of test-time computation on agent robustness, we group all models into two inference categories based on whether explicit reasoning is enabled at inference time.

\textbf{Reasoning Models (Thinking Mode).} 
This group includes models that employ extended chain-of-thought reasoning during inference, including the o-series (o3, o4-mini) and the DeepSeek-R1 family (R1-0528). 
These models are evaluated to assess whether explicit reasoning improves robustness under stochastic user and tool perturbations.

\textbf{Standard Foundation Models (Non-Thinking Mode).} 
This group consists of general-purpose foundation models without explicit reasoning mechanisms at inference time. 
The evaluated models include GPT-4.1 and GPT-5, Claude-4-Sonnet and Claude-4.1-Opus, Gemini-2.5-Flash and Gemini-2.5-Pro, DeepSeek-V3 variants (V3-0324, V3.1, V3.2), the Qwen3 family (32B, 235B-A22B, Max), GLM-4.5, FLM-4.6, Seed-1.6, and LongCat-Flash.

\textbf{Datasets and Noise Protocol.} 
Our evaluation covers six interactive task scenarios drawn from VitaBench and $\tau^2$-Bench, which collectively require multi-turn interaction, tool use, and intent tracking. 
To extend beyond standard agent--user interaction settings, we additionally include solo-agent search tasks adapted from the R1-search framework.

Following prior work, we evaluate agents under non-ideal conditions by introducing stochastic noise into the interaction loop. 
Specifically, we apply noise at two interfaces: 
(1) \textit{user-side noise}, which introduces ambiguous or erroneous instructions; and 
(2) \textit{tool-side noise}, which introduces API failures, latency, or malformed tool outputs. 
This protocol enables systematic analysis of agent failures arising from different stages of the interaction loop.

\textbf{Evaluation Metrics.} 
Each task is executed for $N=4$ independent trials with identical configurations. 
We report Avg@4, defined as the average task success rate across trials, as the primary robustness metric. 
To measure efficiency, we additionally report the average token usage (Avg\_Tokens@4) and the average number of interaction turns (Avg\_Steps@4) required to complete each task.


重新写：既然全是并列写的那么就并列写
Dataset:
为了更全面的评估agent抗噪能力，我们选取了当前agent的两种核心能力：（1）检索，（2）多轮用户agent交互。两种能力对应不同的特性，检索智能适用于工具噪声，多轮用户agent交互则可=可以添加用户噪声和工具噪声。对于检索能力，我们选取Multi-hop QA (2WikiMultiHopQA
(Ho et al., 2020) and HotpotQA (Yang et al., 2018)).对于多轮任务交互，我们选取vitabench和tau2bench。

第二版：
为系统性地评估智能体在复杂环境中的鲁棒性，我们将核心能力划分为两个维度：（1）静态知识检索；（2）动态多轮交互。静态检索任务选用2WikiMultiHopQA（Ho等人，2020）和HotpotQA（Yang等人，2018）两项代表性基准，由于缺乏用户仿真器、仅支持工具调用，故主要引入工具噪声。动态交互任务则选用VitaBench和τ²-Bench两项代表性基准，这两项基准支持同时引入用户噪声与工具噪声。在所有测试领域中，噪声均通过对关键交互接口进行扰动的方式注入，同时严格保持原始任务目标不变。为在覆盖全部预设噪声类型的实验必要性与可扩展性、成本约束之间取得平衡，我们采用分层采样策略：从交互式基准中选取25\%的样本，在多跳问答数据集中选取500个实例。


为系统性地评估智能体在复杂环境中的鲁棒性，我们将核心能力划分为两个维度：（1）静态知识检索 与（2）动态多轮交互。具体而言，针对静态检索任务，我们选用 2WikiMultiHopQA (Ho et al., 2020) 和 HotpotQA (Yang et al., 2018) 两项代表性基准。我们将这两个基准的平均性能统一报告为“检索”指标，用于表征静态知识检索能力。由于此类任务缺乏用户交互，仅涉及工具调用，故主要引入工具噪声。针对动态交互任务，我们则选用 VitaBench 和 τ²-Bench，这两项基准支持同时注入用户噪声与工具噪声。每个维度上，均以原始基准任务作为基础数据集，并通过在其上注入噪声来构建有噪评测实例。在所有测试领域中，噪声均通过对关键交互接口进行扰动的方式引入，同时严格保持原始任务目标不变。
最后，为在覆盖全部噪声类型的全面性与评估的可扩展性、成本约束之间取得平衡，我们采用分层采样策略：从vitabench和τ2-bench每个场景中分别抽取25\%的样本，并从多跳问答数据集中抽取500个实例。这种设计确保了在统一的任务分布下，能够对有噪与无噪环境下的模型性能进行精确对比。

To systematically evaluate agent robustness in complex environments, we delineate core capabilities into two dimensions: (1) static knowledge retrieval and (2) dynamic multi-turn interaction. Specifically, for static retrieval tasks, we employ two representative benchmarks: 2WikiMultiHopQA (Ho et al., 2020) and HotpotQA (Yang et al., 2018). Given that these tasks inherently lack user interaction and solely involve tool calls, we primarily introduce tool noise. Conversely, for dynamic interaction tasks, we utilize VitaBench and $tau^2$-Bench, two benchmarks that support the simultaneous injection of both user noise and tool noise. In each dimension, noisy evaluation instances are constructed by perturbing the original benchmark tasks as base datasets. Across all test domains, noise is introduced by perturbing key interaction interfaces, while strictly preserving the invariance of the original task objectives.

Finally, to strike a balance between the experimental necessity of covering all predefined noise types and the practical constraints of evaluation scalability and cost, we adopt a stratified sampling strategy: 25\% of samples are drawn from each scenario within VitaBench and $	au^2$-Bench, and 500 instances are sampled from the multi-hop QA datasets. This design ensures precise comparative analysis of model performance in both noisy and noise-free environments under a unified task distribution.

==> introduction/intro_backup.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{images/intro.png}
    \vspace{-0.06in}
    \caption{
        Overall scores on AgentNoiseBench.
    }
    \label{fig:intro}
\end{figure*}

\section{Introduction}
Recent advances in large language models (LLMs) have catalyzed a new generation of autonomous agents that can interpret natural-language instructions, perform multi-step planning, and solve tasks in open environments by invoking external tools. Alongside this progress, a growing suite of benchmarks\citep{barres2025tau,he2025vitabench} has been proposed to evaluate agents' task-solving capabilities. While state-of-the-art agents now achieve impressive results on many mainstream benchmarks, an increasing number of evaluations in realistic settings reveal a persistent gap: when tasks move beyond controlled laboratory scenarios into the complex and dynamic real world, even the strongest agents still fall short.

A key reason for this gap is that many existing agent training and evaluation protocols are implicitly grounded in the idealized conditions assumed by standard benchmarks: user instructions are carefully designed, and tool executions are reliable. However, in real deployments, the environment is inherently uncontrolled and noisy. This coupling between objectives and an idealized environment limits systematic exposure to noise and uncertainty, and therefore weakens robustness learning. 

We argue that two noise sources dominate agent failures: (1) instruction-side noise from users, including vague phrasing, missing information, and even logical inconsistencies; and (2) execution-side noise from the environment, such as tool-call failures, incorrect outputs, or unexpected exceptions. Once injected into the action pipeline, these perturbations often trigger cascading errors---misaligned plans, compounding mistakes, and unsuccessful recovery---leading to severe performance degradation or outright task failure. Consequently, agents that score highly on laboratory benchmarks can still deliver poor real-world user experience and fall short of practical requirements for safety and reliability. This motivates the need for evaluation tools and benchmarks that explicitly measure agent robustness and degradation behavior under noisy conditions.

However, systematically evaluating agents under noise is non-trivial, due to three key challenges. First, the community lacks a reusable, principled characterization of noise sources that commonly arise in real deployments---particularly a unified modeling framework that covers both interaction noise from users and feedback noise from tools. Second, noise injection must balance realism with experimental control: it should capture the imperfections encountered in practice, yet remain controllable, reproducible, and easily integrated into the agent's execution pipeline with adjustable strength and plug-and-play design. Third, robustness is inherently multi-dimensional. Final-task success alone rarely explains how and why performance degrades; evaluation should also measure decision stability, sensitivity to perturbations, and resource usage and recovery behaviors under noise, enabling a more diagnostic understanding of failure modes.

To address these challenges, we introduce \textsc{AgentNoiseBench}, a benchmark framework for systematic evaluation of LLM agents' robustness to interaction noise. \textsc{AgentNoiseBench} covers two representative agentic settings: (i) multi-step tool use, targeting DeepSearch-style agents on question answering tasks that require repeated retrieval and evidence aggregation; and (ii) multi-turn human--agent interaction, where we adapt and extend existing interactive benchmarks (e.g., $\tau^2$-Bench and VitaBench) to support controlled injection of user-side noise throughout a dialogue and to measure its impact. \textsc{AgentNoiseBench} models noise from both user instructions and tool outputs. Concretely, we provide a modular noise-injection mechanism that perturbs the agent's execution pipeline at key interaction interfaces---user inputs and tool observations---while allowing fine-grained control over injection location and intensity (e.g., frequency, probability). Beyond final task performance, \textsc{AgentNoiseBench} reports multi-dimensional diagnostic metrics to characterize robustness and degradation behavior, including completion stability, decision consistency, noise-tolerance thresholds, and recovery behavior and resource consumption under noise.

Using \textsc{AgentNoiseBench}, we evaluate 25 tool-augmented models, spanning both thinking and no-thinking LLMs, and conduct a systematic empirical analysis. Our results show that tool-side noise typically induces more severe performance collapse and trajectory drift than user-side noise. Moreover, several strong reasoning models exhibit over-rationalization and repeated verification when faced with incorrect tool feedback, incurring substantial token/step overhead and, in some cases, amplifying erroneous decisions. These findings suggest that evaluation for real-world agents should go beyond ``noise-free success rate'' and treat tool reliability, noise-induced degradation curves, and failure mechanisms as first-class metrics.

In summary, our main contributions are threefold:
\begin{itemize}[leftmargin=*]
  \item \textbf{Benchmark framework.} We introduce \textsc{AgentNoiseBench}, a benchmark for systematic evaluation of agent robustness under interaction noise from both users and tools, covering two representative settings: multi-step tool use and multi-turn interaction.
  \item \textbf{Noise modeling and evaluation protocol.} We propose a deployment-oriented noise modeling and controllable injection mechanism, together with multi-dimensional metrics beyond end-task success to characterize degradation patterns and robustness boundaries.
  \item \textbf{Large-scale empirical study.} We conduct a comprehensive evaluation of 25 tool-using models (including both LLMs and LRMs), identifying key degradation modes and capability gaps under noise, and deriving implications for future agent training and system design.
\end{itemize}

